Unveiling land use dynamics: Insights from a hierarchical Bayesian spatio-temporal modelling of Compositional Data

Changes in land use patterns have significant environmental and socioeconomic impacts, making it crucial for policymakers to understand their causes and consequences. This study, part of the European LAMASUS (Land Management for Sustainability) project, aims to support the EU's climate neutrality target by developing a governance model through collaboration between policymakers, land users, and researchers. We present a methodological synthesis for treating land use data using a Bayesian approach within spatial and spatio-temporal modeling frameworks. The study tackles the challenges of analyzing land use changes, particularly the presence of zero values and computational issues with large datasets. It introduces joint model structures to address zeros and employs sequential inference and consensus methods for Big Data problems. Spatial downscaling models approximate smaller scales from aggregated data, circumventing high-resolution data complications. We explore Beta regression and Compositional Data Analysis (CoDa) for land use data, review relevant spatial and spatio-temporal models, and present strategies for handling zeros. The paper demonstrates the implementation of key models, downscaling techniques, and solutions to Big Data challenges with examples from simulated data and the LAMASUS project, providing a comprehensive framework for understanding and managing land use changes.

==> set_of_notes <==
%% Section 1: Introduction::

% Changes in land-use patterns have important environmental and socioeconomic repercussions. A good understanding of the causes and consequences of these changes would provide neew dimensions to policy making and public policy evaluation.

% Empirical studies of land use changes are very useful to policy-makers who need to be able to identify the determinants of land use changes. Changes in land use patterns significantly impact environmental conditions (biodiversity, water pollution, soil erosion, and climate change) as well as economic and social welfare. These changes are influenced by socioeconomic factors, pedo-climatic factors and policy variables. A good understanding of how these factors influence land use patterns over time and in space would help policy-makers evaluate existing or draw up new public policies that are environmentally friendly.

% Land use plays a vital role in many major societal issues: food security, preservation of biodiversity and ecosystem services and the achievement of many Sustainable Development Goals. Land use choices are the result of complex decision making processes related to the local and global biophysical and socioeconomic drivers. Therefore, land-use models enable to analyse the drivers of land use change and the environmental an socioeconomic impacts of land use change on stakeholders and the whole society. Land use models are also crucial for the design of public policies related to how to feed the growing world population and avoid unwanted land use effects on the environment.

% Various disciplines (economics, statistics, geography, land use science) have developed a range of empirical land use modelling approaches, using either aggregate or individual data. However, most of this work pays little attention to spatial autocorrelation in modelling land use although spatial interdependence is prevalent in all economic decisions in general and in land use decision in particular. As a result, ``standard'' statistical and econometric methods, which assume independent observations, are inappropriate. More generally, taking account of the spatial dimension in econometric models involves two effects: spatial heterogeneity is the spatial differentiation of variables and behaviours in space and usually does not require specific econometric methods. Switching models, semi-parametric modelling of coordinates or clustered robust inference can handle this effect appropriately. Conversely, spatial models refers to the lack of independence among the geographic observations. It measures the degree of similarity between an attribute in one location and the same attribute in neighbouring locations.

% There is a growing body of work on econometric modelling of land use. These studies address the determinants of land use and land use change. Although land use studies taking explicit account of spatial autocorrelation have increased, they remain relatively scarce. Most econometric land use models in papers published in high quality journals still tend to either ignore spatial autocorrelation, or use ad hoc methods to deal with it. This is because the spatial autocorrelation raises several issues related to econometric estimation, hypothesis testing, and prediction. 

%% Section 2: Land use and compositional data::

%% Section 3: Spatial and spatio-temporal models::

% {\color{red}
% % In the previous models we have focused on the spatial component and the association between the point pattern of sampling and the values of the marks. However, these models can be extended by incorporating temporal terms in conjunction with spatial terms, as hinted at earlier. In this subsection, we will provide a brief overview of the different structures that can be encountered in spatio-temporal modelling.

% Spatio-temporal models allow the assessment of spatial and temporal dynamics \citep{Krainski_AdvancedSPDE_2018, Wikle_SpatioTemporalStatistics_2019}, and have been widely used in various fields: in epidemiology \citep{Moraga_MalariaINLA_2021}; in species distribution models \citep{Paradinas_SpatioTemporal_2015, Yuan_PointProcessDistanceSampling_2017}; in models to assess animal movement and habitat preference \citep{Arce_SpatialVariationStepSelection_2023, Michelot_StepSelectionAnalysis_2024}; in econometric models \citep{Virgilio_SpatialEconometricsINLA_2021}; and in many others.

% A comprehensive overview of various additive spatio-temporal structures is provided in \citep{Blangiardo_SpatioTemporalINLA_2013, Paradinas_SpatioTemporal_2017} by decomposing the spatio-temporal term into two distinct components: a pure temporal trend and a pure spatial effect. Depending on their structural characteristics, the following types of structures can be identified: (a) opportunistic spatial distribution, where $u_{st} = w_{st}$, with $w_t \sim \mathcal{N}(\mathbf{0}, \mathbf{Q})$ representing different spatial realisations with consistent hyperparameters across time (essentially replicas of the spatial effect over time); (b) Persistent spatial distribution with random intensity changes over time, expressed as $u_{st} = w_{st} + v_t$, where the spatio-temporal effect is segregated into a spatial trend replicated across time and an independent and identically distributed (i.i.d.) temporal effect $v_t \sim \mathcal{N}(0, \tau_v)$; (c) persistent spatial distribution with temporal intensity trend, where $u_{st}= w_s + v_{t}$, implying the same spatial effect over time and a temporal trend defined by a structured random effect (\textit{rw1}, \textit{rw2}, \textit{ar1}, ...); and finally a (d) progressive spatio-temporal distribution, where the spatio-temporal effect is decomposed as $u_{st} = w_{st} + v_{t}$, with the spatial effect is replicated across time, alongside a structured temporal trend.
% }

% In addition to being able to evaluate spatio-temporal models by decomposing them into two terms, one purely spatial and one purely temporal, it is possible to make a similar synthesis but considering different structures for spatial and temporal interaction components. \cite{KnorrHeld_SpaceTime_2000} proposed four general structures to define spatio-temporal interaction models, in which the precision matrix of the spatio-temporal effect is constructed by means of the Kronecker product of the precision matrix of the spatial component by the precision matrix of the temporal component $\mathbf{Q}_{st}=\mathbf{Q}_s\otimes\mathbf{Q}_t$ \citep{Clayton_GLMM_1996}. According to this approach, four types of interaction emerge naturally by crossing unstructured and structured precision matrices for space and time. 

% Finally, it is also possible to construct non-separable spatio-temporal interaction models \citep{Lindgren_diffusionbased_2024}, i.e. those whose precision matrix can not be decomposed through the Kronecker product of a precision matrix associated to the spatial structure and another one associated to the temporal structure, that is, $\mathbf{Q}_{st} \neq \mathbf{Q}_s \otimes \mathbf{Q}_t$.

%% Section 8: Examples

% \begin{equation}
% \begin{aligned}
% Y_{it} \sim & \text{ Beta}\left(\mu_{it}, \phi \right) \\
% \log \left(\phi\right) = &\ \theta \\
% \text{logit}\left(\mu_{it}\right) = &\ \boldsymbol{\beta} \boldsymbol{X}_{it} + \iint_{s_x, s_y \in C_{i}} \frac{Z(\boldsymbol{s}) ds_x ds_y}{\mid C_i \mid} + \mathcal{U}_t \\
% |C_i| = &\ \iint_{s_x, s_y \in C_{i}} ds_x ds_y \\
% Z(\boldsymbol{s}) \sim &\ \text{GMRF}(0, {Q}(d \mid \rho_u, \sigma_u)) \\
% \mathcal{U}_1 \sim &\ \text{N}(0, (\psi(1 - \rho^2))^{-1}) \\
% \mathcal{U}_t = &\ \rho \cdot \mathcal{U}_{t-1} + \epsilon_t \\
% \epsilon_t \sim &\ \text{N}(0, \psi^{-1}); \quad t = 2, \ldots, n \\
% \theta \sim &\ \text{logGamma}(1, 10^{-5}) \\
% \boldsymbol{\beta} \sim &\ {N} \left(0, 10^{-3}\right) \\
% \rho_u \sim &\ \text{PC-prior}(1, 0.5) \\
% \sigma_u \sim &\ \text{PC-prior}(\rho_u < h, 0.1) \\
% \kappa = &\ \psi(1 - \rho^2) \\
% \textsf{log}(\kappa) = &\ \theta_3 \\
% \textsf{log} \left( \frac{1 + \rho}{1 - \rho} \right) = &\ \theta_4 \\
% \theta_3 \sim &\ \text{logGamma}(1, 5 \cdot 10^{-4}) \\
% \theta_4 \sim &\ \text{N}(0, 0.15), \\
% \end{aligned}
% \end{equation}
% where \( Y_{it} \) represents the random variable denoting the proportion of agricultural land in a specific region \( i \) and year \( t \), with \( i = 1, \ldots, 972 \) and \( t = 1, \ldots, 12 \). The conditional distribution of \( Y_{it} \) follows a Beta distribution with parameters \( \mu_{it} \) and \( \phi \). The mean and precision are linked through the logit and log link functions, respectively. The covariates are represented by \( X_{it} \), and the vector of regression coefficients by \( \boldsymbol{\beta} \). The spatial effect is downscaled, and the temporal effect is modeled as a first-order autoregressive process. For the selection of covariates to include in the model, all possible combinations of models without spatial and temporal effects are considered. The usual measures of fit and predictive quality are computed, and the best model is selected based on the Watanabe–Akaike Information Criterion (WAIC, \citealt{Watanabe_WAIC_2013}). The selected covariates encompass a range of socioeconomic and biophysical characteristics, including general economic indicators and variables related to agricultural policies. Some of the results can be seen in Figure \ref{fig:fig_BetaExample}.
